Schema-Based Query Optimisation for Graph Databases

Recursive graph queries are increasingly popular for extracting information from interconnected data found in various domains such as social networks, life sciences, and business analytics. Graph data often come with schema information that describe how nodes and edges are organized. We propose a type inference mechanism that enriches recursive graph queries with relevant structural information contained in a graph schema. We show that this schema information can be useful in order to improve the performance when evaluating acylic recursive graph queries. Furthermore, we prove that the proposed method is sound and complete, ensuring that the semantics of the query is preserved during the schema-enrichment process.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=main

PDF = $(PACKAGE).pdf
TEX = $(PACKAGE).tex

all:  
	pdflatex ${TEX}
	bibtex $(PACKAGE)
	bibtex $(PACKAGE)
	pdflatex ${TEX}
	pdflatex ${TEX}

%.cls:   %.ins %.dtx
	pdflatex $<

clean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi *.fdb_latexmk *.gz \
	*.fls *.pdf
	
distclean: clean
	$(RM)  *.pdf


